Improved Modeling of $\beta$ Electronic Recoils in Liquid Xenon Using LUX Calibration Data

We report here methods and techniques for creating and improving a model that reproduces the scintillation and ionization response of a dual-phase liquid and gaseous xenon time-projection chamber. Starting with the recent release of the Noble Element Simulation Technique (NEST v2.0), electronic recoil data from the $\beta$ decays of ${}^3$H and ${}^{14}$C in the Large Underground Xenon (LUX) detector were used to tune the model, in addition to external data sets that allow for extrapolation beyond the LUX data-taking conditions. This paper also presents techniques used for modeling complicated temporal and spatial detector pathologies that can adversely affect data using a simplified model framework. The methods outlined in this report show an example of the robust applications possible with NEST v2.0, while also providing the final electronic recoil model and detector parameters that will used in the new analysis package, the LUX Legacy Analysis Monte Carlo Application (LLAMA), for accurate reproduction of the LUX data. As accurate background reproduction is crucial for the success of rare-event searches, such as dark matter direct detection experiments, the techniques outlined here can be used in other single-phase and dual-phase xenon detectors to assist with accurate ER background reproduction.

==> list.tex <==
@article{lux,
      author         = {Akerib \textit{et al.} (LUX Collaboration), D. S.  },
      title          = "{The Large Underground Xenon (LUX) Experiment}",
      collaboration  = "LUX",
      journal        = "Nucl. Instrum. Meth.",
      volume         = "A704",
      year           = "2013",
      pages          = "111-126",
      doi            = "10.1016/j.nima.2012.11.135",
      eprint         = "1211.3788",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
}
\


@article{luxFirst,
  title = "{First Results from the LUX Dark Matter Experiment at the Sanford Underground Research Facility}",
  author = {Akerib \textit{et al.} (LUX Collaboration), D. S.},
  collaboration = {LUX Collaboration},
  journal = {Phys. Rev. Lett.},
  volume = {112},
  issue = {9},
  pages = {091303},
  numpages = {7},
  year = {2014},
  
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.112.091303},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.091303}
}



@article{lux2,
  title = "{Improved Limits on Scattering of Weakly Interacting Massive Particles from Reanalysis of 2013 LUX Data}",
  author = {Akerib \textit{et al.} (LUX Collaboration), D. S.},
  collaboration = {LUX Collaboration},
  journal = {Phys. Rev. Lett.},
  volume = {116},
  issue = {16},
  pages = {161301},
  numpages = {7},
  year = {2016},
 
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.116.161301},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.116.161301}
}

@article{luxRun4,
  title = "{Results from a Search for Dark Matter in the Complete LUX Exposure}",
  author = {Akerib \textit{et al.} (LUX Collaboration), D. S.},
  collaboration = {LUX Collaboration},
  journal = {Phys. Rev. Lett.},
  volume = {118},
  issue = {2},
  pages = {021303},
  numpages = {8},
  year = {2017},
  
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.118.021303},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.118.021303}
}



@article{fieldModeling,
      author         = "Akerib \textit{et al.} (LUX Collaboration), D. S.",
      title          = "{3D Modeling of Electric Fields in the LUX Detector}",
      collaboration  = "LUX",
      journal        = "Journal of Instrumentation",
      volume         = "12",
      year           = "2017",
      number         = "11",
      doi            = "10.1088/1748-0221/12/11/P11022",
      eprint         = "1709.00095",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
}



@article{xenon100_1year,
  title = "{Dark Matter Search Results from a One Ton-Year Exposure of XENON1T}",
  author = {Aprile \textit{et al.} (XENON Collaboration), E.},
  collaboration = {XENON Collaboration  7},
  journal = {Phys. Rev. Lett.},
  volume = {121},
  issue = {11},
  pages = {111302},
  numpages = {8},
  year = {2018},
 
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.121.111302},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.121.111302}
}

@article{pandaX,
  title = "{Dark Matter Results from 54-Ton-Day Exposure of PandaX-II Experiment}",
  author = {Cui \textit{et al.} (PandaX-II Collaboration), Xiangyi},
  collaboration = {PandaX-II Collaboration},
  journal = {Phys. Rev. Lett.},
  volume = {119},
  issue = {18},
  pages = {181302},
  numpages = {7},
  year = {2017},
  
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.119.181302},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.119.181302}
}

@article{TDR,
      author         = "Mount \textit{et al.}, B. J.",
      title          = "{LUX-ZEPLIN (LZ) Technical Design Report}",
      year           = "2017",
      eprint         = "1703.09144",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      reportNumber   = "LBNL-1007256, FERMILAB-TM-2653-AE-E-PPD",
      SLACcitation   = "%%CITATION = ARXIV:1703.09144;%%"
}

@article{LZsens,
      author         = "Akerib \textit{et al.} (LUX-ZEPLIN Collaboration), D. S.",
      title          = "{Projected WIMP Sensitivity of the LUX-ZEPLIN (LZ) Dark
                        Matter Experiment}",
      collaboration  = "LUX-ZEPLIN",
      year           = "2018",
      eprint         = "1802.06039",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      reportNumber   = "FERMILAB-PUB-18-054-AE-PPD",
      SLACcitation   = "%%CITATION = ARXIV:1802.06039;%%"
}

@article{jonC14,
      author         = "Akerib \textit{et al.} (LUX Collaboration), D. S.",
      title          = "{Improved Measurements of the $\beta$-Decay Response of
                        Liquid Xenon with the LUX Detector}",
      collaboration  = "LUX",
      year           = "2019",
      eprint         = "1903.12372",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
} 

@article{tritium,
      author         = "Akerib \textit{et al.} (LUX Collaboration), D. S.",
      title          = "{Tritium calibration of the LUX dark matter experiment}",
      collaboration  = "LUX",
      journal        = "Phys. Rev.",
      volume         = "D93",
      year           = "2016",
      number         = "7",
      pages          = "072009",
      doi            = "10.1103/PhysRevD.93.072009",
      eprint         = "1512.03133",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
}

@article{nest1,
	doi = {10.1088/1748-0221/6/10/p10002},
	year = 2011,
	
	publisher = {{IOP} Publishing},
	volume = {6},
	number = {10},
	pages = {P10002},
	author = {Szydagis \textit{et al.}, M.},
	title = {{NEST}: a comprehensive model for scintillation yield in liquid xenon},
	journal = {Journal of Instrumentation}
}

@article{nest2013,
	doi = {10.1088/1748-0221/8/10/c10003},
	year = 2013,

	publisher = {{IOP} Publishing},
	volume = {8},
	number = {10},
	pages = {C10003},
	author = {Szydagis \textit{et al.}, M.},
	title = "{Enhancement of {NEST} capabilities for simulating low-energy recoils in liquid xenon}",
	journal = {Journal of Instrumentation}
}

@article{Doke,
	doi = {10.1143/jjap.41.1538},
	url = {https://doi.org/10.11432Fjjap.41.1538},
	year = 2002,
	
	publisher = {Japan Society of Applied Physics},
	volume = {41},
	number = {Part 1, No. 3A},
	pages = {1538--1545},
	author = {Doke \textit{et al.}, T.},
	title = "{Absolute Scintillation Yields in Liquid Argon and Xenon for Various Particles}",
	journal = {Japanese Journal of Applied Physics}
}

@article{SignalYields,
  title = "{Signal yields, energy resolution, and recombination fluctuations in liquid xenon}",
  author = {Akerib \textit{et al.} (LUX Collaboration), D. S.},
  collaboration = {LUX Collaboration},
  journal = {Phys. Rev. D},
  volume = {95},
  issue = {1},
  numpages = {12},
  year = {2017},
  
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.95.012008},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.95.012008}
}

@article{Conti,
      author         = "Conti \textit{et al.}, E.",
      title          = "{Correlated fluctuations between luminescence and
                        ionization in liquid xenon}",
      collaboration  = "EXO-200",
      journal        = "Phys. Rev.",
      volume         = "B68",
      year           = "2003",
      pages          = "054201",
      doi            = "10.1103/PhysRevB.68.054201",
      eprint         = "hep-ex/0303008",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "SLAC-PUB-10181"
}

@phdthesis{JonThesis,
  author       = {Balajthy, J.}, 
  title        = "{Purity Monitoring Techniques and Electronic Energy Deposition Properties in Liquid Xenon Time Projection Chambers}",
  school       = {University of Maryland},
  doi = {https://doi.org/10.13016/M2BG2HD6T},
  year         = 2018
}

@phdthesis{AttilaThesis,
  author       = {Dobi, A.}, 
  title        = "{Measurement of the Electron Recoil Band of the LUX Dark Matter Detector With a Tritium Calibration Source}",
  school       = {University of Maryland},
  year         = 2018
}

@phdthesis{DahlThesis,
      author         = "Dahl, C. E.",
      title          = "{The physics of background discrimination in liquid
                        xenon, and first results from XENON10 in the hunt for WIMP
                        dark matter}",
      school         = "Princeton U.",
      year           = "2009",
      url            = "https://www.princeton.edu/physics/graduate-program/theses/theses-from-2009/E.Dahlthesis.pdf",
      reportNumber   = "AAT-3364532",
}

@article{neriX,
      author         = "Goetzke \textit{et al.} (Columbia U.), L. W",
      title          = "{Measurement of light and charge yield of low-energy
                        electronic recoils in liquid xenon}",
      journal        = "Phys. Rev.",
      volume         = "D96",
      year           = "2017",
      number         = "10",
      pages          = "103007",
      doi            = "10.1103/PhysRevD.96.103007",
      eprint         = "1611.10322",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
}


@article{Aprile2012,
      author         = "Aprile \textit{et al.} (XENON Collaboration), E.",
      title          = "{Dark Matter Results from 225 Live Days of XENON100
                        Data}",
      collaboration  = "XENON100",
      journal        = "Phys. Rev. Lett.",
      volume         = "109",
      year           = "2012",
      pages          = "181301",
      doi            = "10.1103/PhysRevLett.109.181301",
      eprint         = "1207.5988",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
}


@article{pixey,
      author         = "Boulton \textit{et al.}, E. M.",
      title          = "{Calibration of a two-phase xenon time projection chamber
                        with a $^{37}$Ar source}",
      journal        = "Journal of Instrumentation",
      volume         = "12",
      year           = "2017",
      number         = "08",
      pages          = "P08004",
      doi            = "10.1088/1748-0221/12/08/P08004",
      eprint         = "1705.08958",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
}

@article{LUX_xe127,
      author         = "Akerib \textit{et al.} (LUX Collaboration), D. S",
      title          = "{Ultralow energy calibration of LUX detector using
                        $^{127}$Xe electron capture}",
      collaboration  = "LUX",
      journal        = "Phys. Rev.",
      volume         = "D96",
      year           = "2017",
      number         = "11",
      pages          = "112011",
      doi            = "10.1103/PhysRevD.96.112011",
      eprint         = "1709.00800",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
}

@article{lin,
  title = "{Scintillation and ionization responses of liquid xenon to low energy electronic and nuclear recoils at drift fields from 236 V/cm to 3.93 kV/cm}",
  author = {Lin \textit{et al.}, Qing},
  journal = {Phys. Rev. D},
  volume = {92},
  issue = {3},
  pages = {032005},
  numpages = {9},
  year = {2015},
  
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.92.032005},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.92.032005}
}

@article{Akimov_2016,
	doi = {10.1088/1748-0221/11/03/c03007},
	url = {https://doi.org/10.1088%2F1748-0221%2F11%2F03%2Fc03007},
	year = 2016,
	
	publisher = {{IOP} Publishing},
	volume = {11},
	number = {03},
	pages = {C03007},
	author = {D.Yu. Akimov and others},
	title = {Observation of delayed electron emission in a two-phase liquid xenon detector},
	journal = {Journal of Instrumentation},
	
}

@article{XENON10,
title = "{Design and performance of the XENON10 dark matter experiment}",
journal = "Astroparticle Physics",
volume = "34",
number = "9",
pages = "679 - 698",
year = "2011",
issn = "0927-6505",
doi = "https://doi.org/10.1016/j.astropartphys.2011.01.006",
url = "http://www.sciencedirect.com/science/article/pii/S0927650511000089",
author = "E. Aprile and others",
}

@article{zepIII,
      author         = "Lebedenko \textit{et al.}, V. N.",
      title          = "{Result from the First Science Run of the ZEPLIN-III Dark
                        Matter Search Experiment}",
      journal        = "Phys. Rev.",
      volume         = "D80",
      year           = "2009",
      pages          = "052010",
      doi            = "10.1103/PhysRevD.80.052010",
      eprint         = "0812.1150",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph"
}

@article{DB,
      author         = "Doke \textit{et al.}, T.",
      title          = "{Let Dependence of Scintillation Yields in Liquid Argon}",
      journal        = "Nucl. Instrum. Meth.",
      volume         = "A269",
      year           = "1988",
      pages          = "291-296",
      doi            = "10.1016/0168-9002(88)90892-3",
}

@article{TIB,
  title = {Recombination of electron-ion pairs in liquid argon and liquid xenon},
  author = {Thomas, J. and Imel, D. A.},
  journal = {Phys. Rev. A},
  volume = {36},
  issue = {2},
  pages = {614--616},
  numpages = {0},
  year = {1987},
  
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.36.614},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.36.614}
}


@article{pixey1,
	doi = {10.1088/1748-0221/13/01/p01005},
	url = {https://doi.org/10.1088\%2F1748-0221\%2F13\%2F01\%2Fp01005},
	year = 2018,
	
	publisher = {{IOP} Publishing},
	volume = {13},
	number = {01},
	pages = {P01005},
	author = {B.N.V. Edwards \textit{et al.}},
	title = {Extraction efficiency of drifting electrons in a two-phase xenon time projection chamber},
	journal = {Journal of Instrumentation},
}

@misc{nestv2,
  author       = {Szydagis \textit{et al.}, M.},
  title        = "{Noble Element Simulation Technique v2.0 (10.5281/zenodo.1314669)}", 
  year         = 2018,
  doi          = {(10.5281/zenodo.1314669)},
  journal          = {https://doi.org/10.5281/zenodo.1314669}
}


@article{SEfit,
      author         = "Chepel, V. and Araujo, H.",
      title          = "{Liquid noble gas detectors for low energy particle
                        physics}",
      journal        = "Journal of Instrumentation",
      volume         = "8",
      year           = "2013",
      pages          = "R04001",
      doi            = "10.1088/1748-0221/8/04/R04001",
      eprint         = "1207.2292",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
     
}


@book{nobelBook,
      author         = "Aprile, Elena and Bolotnikov, Aleksey E. and Bolozdynya,
                        Alexander L. and Doke, Tadayoshi",
      title          = "{Noble Gas Detectors}",
      publisher      = "Wiley",
      year           = "2008",
      doi            = "10.1002/9783527610020",
      ISBN           = "9783527405978, 9783527610020",
}

@article{xenonNtData,
      author         = "Aprile \textit{et al.} (XENON Collaboration), E. ",
      title          = "{XENON1T dark matter data analysis: Signal and background
                        models and statistical inference}",
      collaboration  = "XENON",
      journal        = "Phys. Rev.",
      volume         = "D99",
      year           = "2019",
      number         = "11",
      pages          = "112009",
      doi            = "10.1103/PhysRevD.99.112009",
      eprint         = "19tex02.11297",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",

}

@article{axionLUX,
      author         = "Akerib \textit{et al.} (LUX Collaboration), D. S. ",
      title          = "{First Searches for Axions and Axionlike Particles with
                        the LUX Experiment}",
      collaboration  = "LUX",
      journal        = "Phys. Rev. Lett.",
      volume         = "118",
      year           = "2017",
      number         = "26",
      pages          = "261301",
      doi            = "10.1103/PhysRevLett.118.261301",
      eprint         = "1704.02297",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",

}

@article{mirrorDM,
      author         = "Akerib \textit{et al.} (LUX Collaboration), D. S. ",
      title          = "{First direct detection constraint on mirror dark matter
                        kinetic mixing using LUX 2013 data}",
      collaboration  = "LUX",
      year           = "2019",
      eprint         = "1908.03479",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
}bib
